Towards a Scalable In Situ Fast Fourier Transform

The Fast Fourier Transform (FFT) is a numerical operation that transforms a function into a form comprised of its constituent frequencies and is an integral part of scientific computation and data analysis. The objective of our work is to enable use of the FFT as part of a scientific in situ processing chain to facilitate the analysis of data in the spectral regime. We describe the implementation of an FFT endpoint for the transformation of multi-dimensional data within the SENSEI infrastructure. Our results show its use on a sample problem in the context of a multi-stage in situ processing workflow.

==> notes.tex <==

Additional references not included

=================
https://www.hpcwire.com/2020/07/15/heffte-highly-efficient-fft-for-exascale/

Overview piece from HPCWire about the heFFTe article

=================
https://link.springer.com/chapter/10.1007/978-3-030-50371-0_19#citeas

Link to abstract and to ICCS 2020 confc proceedings PDF from Springer


https://icl.utk.edu/fft/
heFFTe webpage
includes links to github repo, more papers


=================

https://link.springer.com/content/pdf/10.1007/s00034-019-01136-8.pdf?pdf=button

50 Years of FFT Algorithms and Applications

G. Ganesh Kumar 1 · Subhendu K. Sahoo 1 · Pramod Kumar Meher 2

Abstract
The fast Fourier transform (FFT) algorithm was developed by Cooley and Tukey
in 1965. It could reduce the computational complexity of discrete Fourier transform
significantly from O(N 2) to O(N log 2 N ). The invention of FFT is considered as a
landmark development in the field of digital signal processing (DSP), since it could
expedite the DSP algorithms significantly such that real-time digital signal processing
could be possible. During the past 50 years, many researchers have contributed to
the advancements in the FFT algorithm to make it faster and more efficient in order
to match with the requirements of various applications. In this article, we present a
brief overview of the key developments in FFT algorithms along with some popular
applications in speech and image processing, signal analysis, and communication
systems.
